UPL: Uncertainty-aware Pseudo-labeling for Imbalance Transductive Node Classification

Graph-structured datasets often suffer from class imbalance, which complicates node classification tasks. In this work, we address this issue by first providing an upper bound on population risk for imbalanced transductive node classification. We then propose a simple and novel algorithm, Uncertainty-aware Pseudo-labeling (UPL). Our approach leverages pseudo-labels assigned to unlabeled nodes to mitigate the adverse effects of imbalance on classification accuracy. Furthermore, the UPL algorithm enhances the accuracy of pseudo-labeling by reducing training noise of pseudo-labels through a novel uncertainty-aware approach. We comprehensively evaluate the UPL algorithm across various benchmark datasets, demonstrating its superior performance compared to existing state-of-the-art methods.

==> Results/Log/num_augmentation.tex <==
\begin{table}
\vspace{-1em}
\caption{\small Experimental results of Ablation study of our proposed algorithm. All the experiments have been done using the GCN architecture. We report the averaged balanced accuracy, averaged F1-score and the standard error of each experiment for Cora, CiteSeer and PubMed datasets.}
\begin{center}

\begin{scriptsize}
\setlength{\columnsep}{1pt}%
\centering
  \resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}rlcc|cc|cc@{}}
\toprule
 & \textbf{Dataset} & \multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{CiteSeer} & \multicolumn{2}{c}{PubMed}  \\ 
\cline{1-8}\rule{0pt}{2.2ex}
& \textbf{Imbalance Ratio ($\rho=10$)} & bAcc. & F1 & bAcc. & F1 & bAcc. & F1 \\
\cline{1-8}
\rule{0pt}{2.5ex}  
                     
                     % 0
                     & 200 
                     & 74.77 \tiny{$\pm 0.91$} & 73.95 \tiny{$\pm 0.99$}
                     & 67.57 \tiny{$\pm 0.76$} & 67.27 \tiny{$\pm 0.73$}
                     & 74.14 \tiny{$\pm 0.63$} & 73.27 \tiny{$\pm 0.69$} \\
                    % 2
                     & 1000
                     & 75.60 \tiny{$\pm 0.85$} & 74.36 \tiny{$\pm 0.90$}
                     & 69.48 \tiny{$\pm 0.29$} & 69.35 \tiny{$\pm 0.26$}
                     & 74.47 \tiny{$\pm 0.48$} & 74.12 \tiny{$\pm 0.59$} \\
\bottomrule
\end{tabular}}

\end{scriptsize}
\end{center}
\label{tb:augmentation_comparresion}
\end{table}
\vspace{-0.05in}

==> Results/nips/Ablation_hetero.tex <==
% \begin{table*}[htp!]
% \caption{\small Experimental results of our Ablation study of our proposed algorithm. All the experiments have been done using the GCN architecture. We report the averaged balanced accuracy, averaged F1-score and the standard error of each experiment for Cora, CiteSeer and PubMed datasets.}
% \label{tb:Ablation_heterosa}
% \begin{center}
% \begin{scriptsize}
% \setlength{\columnsep}{1pt}%
%  \resizebox{0.9\textwidth}{!}{
% \begin{tabular}{@{}rlcc|cc|cc@{}}
% \toprule
%  & \textbf{Dataset} & \multicolumn{2}{c}{Chameleon} & \multicolumn{2}{c}{Squirrel} & \multicolumn{2}{c}{Wisconsin}  \\ 
% \cline{1-8}\rule{0pt}{2.2ex}
% & \textbf{\makecell{Imbalance Ratio\\ ($\rho=10$)}} & bAcc. & F1 & bAcc. & F1 & bAcc. & F1 \\
% \cline{1-8}
% \rule{0pt}{2.5ex}  

                                        
%                      % 0
%                      & Vanilla 
%                      & 57.01 \tiny{$\pm 0.53$} & 55.61 \tiny{$\pm 0.67$}
%                      & 38.07 \tiny{$\pm 0.57$} & 34.81 \tiny{$\pm 0.69$}
%                      & 34.51 \tiny{$\pm 2.31$} & 31.45 \tiny{$\pm 2.66$} \\
%                     % 2
%                      & + BS
%                      & 58.60 \tiny{$\pm 1.06$} & 58.20 \tiny{$\pm 1.00$}
%                      & 41.81 \tiny{$\pm 0.64$} & 41.27 \tiny{$\pm 0.71$}
%                      & \textbf{44.44} \tiny{$\pm 3.46$} & \textbf{41.29} \tiny{$\pm 2.85$} \\
%                     %4
%                      & + RKC
%                      & 57.18 \tiny{$\pm 0.75$} & 55.84 \tiny{$\pm 0.81$}
%                      & 38.16 \tiny{$\pm 0.54$} & 35.21 \tiny{$\pm 0.55$}
%                      & 35.92 \tiny{$\pm 1.69$} & 32.84 \tiny{$\pm 1.66$} \\
%                     % 5
%                      & + UPL
%                      & 59.64 \tiny{$\pm 0.76$} & 58.77 \tiny{$\pm 0.84$}
%                      & 41.25 \tiny{$\pm 0.55$} & 39.81 \tiny{$\pm 0.58$}
%                      & 34.90 \tiny{$\pm 1.60$} & 31.90 \tiny{$\pm 1.71$} \\
%                     % % 6
%                     %  & + PL - Uncertainty
%                     %  & 60.29 \tiny{$\pm 0.92$} & 59.36 \tiny{$\pm 1.06$}
%                     %  & 41.58 \tiny{$\pm 0.36$} & 39.75 \tiny{$\pm 0.50$}
%                     %  & -- \tiny{$\pm -$} & -- \tiny{$\pm -$} \\
%                     % 7
%                      & + BS + RKC 
%                      & 59.06 \tiny{$\pm 0.90$} & 58.51 \tiny{$\pm 0.95$}
%                      & 41.13 \tiny{$\pm 0.32$} & 40.57 \tiny{$\pm 0.41$}
%                      & 41.97 \tiny{$\pm 3.41$} & 39.26 \tiny{$\pm 2.66$} \\
%                     % 8
%                      & + BS + UPL 
%                      & \underline{60.91} \tiny{$\pm 0.66$} & \underline{60.37} \tiny{$\pm 0.62$}
%                      & \underline{41.58} \tiny{$\pm 0.51$} & \underline{41.35} \tiny{$\pm 0.55$}
%                      & \underline{44.03} \tiny{$\pm 2.25$} & \underline{39.57} \tiny{$\pm 2.09$} \\
%                      % % 9
%                      % & + BS + PL - Uncertainty
%                      % & 61.82 \tiny{$\pm 0.90$} & 61.35 \tiny{$\pm 0.87$}
%                      % & 41.29 \tiny{$\pm 0.49$} & 40.97 \tiny{$\pm 0.51$}
%                      % & -- \tiny{$\pm -$} & -- \tiny{$\pm -$} \\
%                     % 10    
%                      & + UPL + RKC 
%                      & 59.76 \tiny{$\pm 0.65$} & 58.88 \tiny{$\pm 0.77$}
%                      & 41.40 \tiny{$\pm 0.42$} & 39.78 \tiny{$\pm 0.45$}
%                      & 36.17 \tiny{$\pm 1.68$} & 33.25 \tiny{$\pm 1.16$} \\
%                     \cdashline{2-8}
%                      & UPR 
%                      & \textbf{60.97} \tiny{$\pm 0.83$} & \textbf{60.44} \tiny{$\pm 0.78$}
%                      & \textbf{41.98} \tiny{$\pm 0.36$} & \textbf{41.55} \tiny{$\pm 0.38$}
%                      & 36.55 \tiny{$\pm 1.57$} & 33.56 \tiny{$\pm 1.11$} \\
                     
% \bottomrule
% \end{tabular}}

% \end{scriptsize}
% \end{center}
% \end{table*}

% \vspace{-0.05in}

==> Results/nips/Integration_hetero.tex <==










\begin{table*}[htp!]
\caption{\small Further experiments using our Regularization method (RKC) and other baselines on three class-imbalanced heterophilic datasets: Chameleon, Squirrel and Wisconsin. All other settings are similar to the result table of homophilic datasets.}
\begin{center}
\begin{scriptsize}
\setlength{\columnsep}{1pt}%
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{@{\extracolsep{1pt}}rlcc|cc|cc@{}}
\toprule
 & \multirow{1}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{Chameleon} & \multicolumn{2}{c}{Squirrel} & \multicolumn{2}{c}{Wisconsin}  \\ 
\cline{2-8}\rule{0pt}{2.2ex}
& \textbf{Imbalance Ratio ($\rho=10$)} & bAcc. & F1 & bAcc. & F1 & bAcc. & F1 \\
\cline{2-8}
\rule{0pt}{2.5ex}  
\multirow{8}{*}{\rotatebox{90}{GCN}} 
    
                    \rule{0pt}{2ex}
                    % & Re-Weight 
                    %   & 36.07 \tiny{$\pm 0.87$}& 35.61 \tiny{$\pm 0.81$}
                    
                    %  & 26.92 \tiny{$\pm 0.53$}& 25.04 \tiny{$\pm 0.59$}
                     
                    %  & 44.13 \tiny{$\pm 3.08$}& 40.74 \tiny{$\pm 3.27$}
                    %  \\
                    
                    %  & PC Softmax 
                    %   & 36.86 \tiny{$\pm 1.04$}& 36.24 \tiny{$\pm 1.01$}
                    
                    %  & 26.49 \tiny{$\pm 0.59$}& 25.73 \tiny{$\pm 0.49$}
                     
                    %  & 30.90 \tiny{$\pm 3.10$}& 28.15 \tiny{$\pm 2.16$}
                    %  \\
                     
                    %  & DR-GCN 
                    %  & 33.34 \tiny{$\pm 0.81$}& 29.60 \tiny{$\pm 0.79$}
                     
                    %  & 23.34 \tiny{$\pm 0.43$}& 18.20 \tiny{$\pm 0.49$}
                     
                    %  & 29.44 \tiny{$\pm 1.36$}& 27.08 \tiny{$\pm 1.37$}
                    %  \\
                     
                     & GraphSMOTE 
                     & 52.38 \tiny{$\pm 0.77$}& 50.03 \tiny{$\pm 0.76$}
                     & 41.30 \tiny{$\pm 0.47$}& 39.07 \tiny{$\pm 0.60$}
                     & 45.36 \tiny{$\pm 4.21$}& 40.91 \tiny{$\pm 4.39$} \\


                     & +\textbf{RKC}
                     & \textbf{52.88} \tiny{$\pm 0.64$}& \textbf{50.44} \tiny{$\pm 0.72$}
                     & \textbf{41.41} \tiny{$\pm 0.38$}& \textbf{39.21} \tiny{$\pm 0.49$}
                     & \textbf{43.39} \tiny{$\pm 2.11$}& \textbf{44.26} \tiny{$\pm 2.21$} \\

                     \cline{2-8}
                     
                     & Vanilla  
                     & 44.99 \tiny{$\pm 0.87$} & 37.34 \tiny{$\pm 1.33$} 
                     & 31.55 \tiny{$\pm 0.24$} & 23.76 \tiny{$\pm 0.21$} 
                     & 37.27 \tiny{$\pm 1.45$} & 33.14 \tiny{$\pm 0.97$} \\
                     % & + \textbf{TAM}
                     % & 33.02 \tiny{$\pm 0.32$} & 25.23 \tiny{$\pm 0.31$} & 27.23 \tiny{$\pm 0.28$} & 19.59 \tiny{$\pm 0.33$} & 39.75 \tiny{$\pm 2.05$} & 34.12 \tiny{$\pm 1.43$} \\
                     & + \textbf{RKC}
                     & \textbf{53.16} \tiny{$\pm 0.51$} & \textbf{52.36} \tiny{$\pm 0.56$} & \textbf{37.21} \tiny{$\pm 0.42$} & \textbf{35.20} \tiny{$\pm 0.50$} & \textbf{48.75} \tiny{$\pm 2.23$} & \textbf{43.04} \tiny{$\pm 1.49$} \\
                     % & + \textbf{TAM} + \textbf{RKC}
                     % & 33.56 \tiny{$\pm 0.47$} & 27.22 \tiny{$\pm 0.81$} & 26.52 \tiny{$\pm 0.37$} & 20.37 \tiny{$\pm 0.34$} & 42.83 \tiny{$\pm 1.89$} & 36.60 \tiny{$\pm 1.13$} \\
                     \cdashline{2-8}
                     & BalancedSoftmax  
                     & 55.21 \tiny{$\pm 1.99$} & 55.07 \tiny{$\pm 2.10$} 
                     & 39.17 \tiny{$\pm 0.35$} & 37.35 \tiny{$\pm 0.49$} 
                     & 47.93 \tiny{$\pm 1.89$} & 41.75 \tiny{$\pm 1.19$} \\
                     % & + \textbf{TAM}
                     % & 33.28 \tiny{$\pm 0.41$} & 27.28 \tiny{$\pm 0.56$} 
                     % & 27.46 \tiny{$\pm 0.33$} & 20.83 \tiny{$\pm 0.37$} 
                     % & \textbf{48.83} \tiny{$\pm 0.33$} & 40.74 \tiny{$\pm 1.29$} \\
                     & + \textbf{RKC}
                     & \textbf{55.16} \tiny{$\pm 0.54$} & \textbf{55.34} \tiny{$\pm 0.56$} 
                     & \textbf{40.03} \tiny{$\pm 0.21$} & \textbf{38.19} \tiny{$\pm 0.33$} 
                     & \textbf{48.67} \tiny{$\pm 2.03$} & \textbf{41.77} \tiny{$\pm 1.49$} \\
                     % & + \textbf{TAM} + \textbf{RKC}
                     % & 34.10 \tiny{$\pm 0.51$} & 27.90 \tiny{$\pm 0.59$} 
                     % & 26.94 \tiny{$\pm 0.38$} & 21.07 \tiny{$\pm 0.40$} 
                     % & 47.83 \tiny{$\pm 2.13$} & 39.53 \tiny{$\pm 1.36$} \\
                     \cdashline{2-8}
                     & GraphENS 
                     & \textbf{56.89} \tiny{$\pm 0.41$} & \textbf{56.87} \tiny{$\pm 0.43$} 
                     & 36.78 \tiny{$\pm 0.46$} & \textbf{35.95} \tiny{$\pm 0.48$} 
                     & 44.17 \tiny{$\pm 2.13$} & 39.38 \tiny{$\pm 1.65$} \\
                     % & + \textbf{TAM}
                     % & 41.33 \tiny{$\pm 0.62$} & 38.86 \tiny{$\pm 0.78$} 
                     % & 26.94 \tiny{$\pm 0.47$} & 22.41 \tiny{$\pm 0.69$} 
                     % & 42.96 \tiny{$\pm 2.49$} & 38.43 \tiny{$\pm 1.66$} \\
                     & + \textbf{RKC}
                     & \textbf{56.89} \tiny{$\pm 0.45$} & 56.84 \tiny{$\pm 0.42$} 
                     & \textbf{36.79} \tiny{$\pm 0.36$} & 35.84 \tiny{$\pm 0.35$} 
                     & \textbf{45.46} \tiny{$\pm 2.53$} & \textbf{40.97} \tiny{$\pm 1.90$} \\
                     % & + \textbf{TAM} + \textbf{RKC}
                     % & 42.41 \tiny{$\pm 0.54$} & 40.27 \tiny{$\pm 0.75$} 
                     % & 27.96 \tiny{$\pm 0.50$} & 23.31 \tiny{$\pm 0.66$} 
                     % & 44.26 \tiny{$\pm 2.47$} & 39.73 \tiny{$\pm 1.76$} \\
\bottomrule
\end{tabular}
}
\end{scriptsize}
\end{center}
\label{tb:integration_hetro}
\vspace{-0.05in}
\end{table*}


==> Results/nips/Integration_homo.tex <==

\begin{table*}[htp!]
\caption{\small Experimental results of our Regularization method (RKC) and other baselines on three class-imbalanced node classification benchmark datasets: Cora, CiteSeer and PubMed. We report averaged balanced accuracy (bAcc.) and F1-score with the standard errors for 10 repetitions on GCN model.}
\begin{center}
\begin{scriptsize}
\setlength{\columnsep}{1pt}%
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{@{\extracolsep{1pt}}rlcc|cc|cc@{}}
\toprule
 & \multirow{1}{*}{\textbf{Dataset}} & \multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{CiteSeer} & \multicolumn{2}{c}{PubMed}  \\ 
\cline{2-8}\rule{0pt}{2.2ex}
& \textbf{Imbalance Ratio ($\rho=10$)} & bAcc. & F1 & bAcc. & F1 & bAcc. & F1 \\
\cline{2-8}
\rule{0pt}{2.5ex}  
\multirow{8}{*}{\rotatebox{90}{GCN}} 
    
                    \rule{0pt}{2ex}
                     % & Re-Weight
                     % & 65.52 \tiny{$\pm 0.84$}& 65.54 \tiny{$\pm 1.20$}
                     % & 44.52 \tiny{$\pm 1.22$}& 38.85 \tiny{$\pm 1.62$}
                     % & 70.17 \tiny{$\pm 1.25$}& 66.37 \tiny{$\pm 1.73$}
                     % \\
                    
                     % & PC Softmax 
                     % & 67.79 \tiny{$\pm 0.92$}& 67.39 \tiny{$\pm 1.08$}
                     % & 49.81 \tiny{$\pm 1.12$}& 45.55 \tiny{$\pm 1.26$}
                     % & 70.20 \tiny{$\pm 0.60$}& 68.83 \tiny{$\pm 0.73$}
                     % \\
                     
                     % & DR-GCN 
                     % & 60.17 \tiny{$\pm 0.83$}& 59.31 \tiny{$\pm 0.97$}
                     % & 42.64 \tiny{$\pm 0.75$}& 38.22 \tiny{$\pm 1.22$}
                     % & 65.51 \tiny{$\pm 0.81$}& 64.95 \tiny{$\pm 0.53$}
                     % \\
                     
                     % \cline{2-8}
              
                     & GraphSMOTE 
                     & 62.66 \tiny{$\pm 0.83$} & 61.76 \tiny{$\pm 0.96$}
                     & 34.26 \tiny{$\pm 0.89$} & 28.31 \tiny{$\pm 1.48$}
                     & 68.94 \tiny{$\pm 0.89$} & 64.17 \tiny{$\pm 1.43$}\\
                     & + \textbf{RKC}
                     & \textbf{66.18} \tiny{$\pm0.82$} & \textbf{64.83} \tiny{$\pm 0.97$} 
                     & \textbf{40.37} \tiny{$\pm1.72$} & \textbf{39.51} \tiny{$\pm 1.73$} 
                     & \textbf{72.73} \tiny{$\pm0.54$} & \textbf{72.40} \tiny{$\pm 0.58$} \\
                     \cdashline{2-8}
                     
                     & Vanila
                     & 52.57 \tiny{$\pm 0.38$} & 43.66 \tiny{$\pm 0.75$} 
                     & 35.33 \tiny{$\pm 0.17$} & 23.01 \tiny{$\pm 0.15$} 
                     & 63.60 \tiny{$\pm 0.09$} & 47.93 \tiny{$\pm 0.10$} \\
                     % & + \textbf{TAM}
                     % & 52.00 \tiny{$\pm 0.40$} & 42.81 \tiny{$\pm 0.75$} 
                     % & 33.16 \tiny{$\pm 0.18$} & 22.13 \tiny{$\pm 0.20$} 
                     % & 64.20 \tiny{$\pm 0.24$} & 49.11 \tiny{$\pm 0.43$} \\
                     & + \textbf{RKC}
                     & \textbf{59.07} \tiny{$\pm 1.22$} & \textbf{53.74} \tiny{$\pm 1.91$} 
                     & \textbf{54.46} \tiny{$\pm 1.06$} & \textbf{51.41} \tiny{$\pm 1.38$} 
                     & \textbf{70.04} \tiny{$\pm 0.48$} & \textbf{71.39} \tiny{$\pm 0.48$} \\
                     \cdashline{2-8}
                     
                     & BalancedSoftmax 
                     & 64.90 \tiny{$\pm 1.05$} & 61.23 \tiny{$\pm 1.28$} 
                     & 51.13 \tiny{$\pm 1.00$} & 46.66 \tiny{$\pm 1.30$} 
                     & 69.33 \tiny{$\pm 0.68$} & 63.71 \tiny{$\pm 1.42$} \\
                     % & + \textbf{TAM}
                     % & 63.09 \tiny{$\pm 1.10$} & 59.48 \tiny{$\pm 1.34$} 
                     % & 38.89 \tiny{$\pm 2.01$} & 31.96 \tiny{$\pm 2.72$} 
                     % & 67.83 \tiny{$\pm 1.24$} & 59.61 \tiny{$\pm 2.29$} \\
                     & + \textbf{RKC}
                     & \textbf{67.22} \tiny{$\pm 0.73$} & \textbf{64.25} \tiny{$\pm 0.88$} 
                     & \textbf{55.90} \tiny{$\pm 0.87$} & \textbf{53.28} \tiny{$\pm 1.14$} 
                     & \textbf{72.98} \tiny{$\pm 0.52$} & \textbf{72.89} \tiny{$\pm 0.76$} \\
                     % & + \textbf{TAM} + \textbf{RKC}
                     % & 61.59 \tiny{$\pm 1.22$} & 59.42 \tiny{$\pm 1.23$} 
                     % & 44.88 \tiny{$\pm 2.06$} & 40.03 \tiny{$\pm 2.78$} 
                     % & 67.70 \tiny{$\pm 1.04$} & 61.69 \tiny{$\pm 2.06$} \\
                     \cdashline{2-8}
                     
                     & GraphENS 
                     & 69.69 \tiny{$\pm 0.52$} & 69.77 \tiny{$\pm 0.60$} 
                     & 53.62 \tiny{$\pm 1.12$} & 50.08 \tiny{$\pm 1.39$} 
                     & 71.15 \tiny{$\pm 0.80$} & 67.92 \tiny{$\pm 1.15$} \\
                     % & + \textbf{TAM}
                     % & 69.95 \tiny{$\pm 0.70$} & 70.16 \tiny{$\pm 0.68$} 
                     % & 56.01 \tiny{$\pm 0.80$} & 54.83 \tiny{$\pm 0.98$} 
                     % & 71.35 \tiny{$\pm 0.77$} & 68.81 \tiny{$\pm 1.31$} \\
                     & + \textbf{RKC}
                     & \textbf{72.32} \tiny{$\pm 0.62$} & \textbf{71.57} \tiny{$\pm 0.62$} 
                     & \textbf{57.47} \tiny{$\pm 0.93$} & \textbf{55.98} \tiny{$\pm 1.03$} 
                     & \textbf{72.89} \tiny{$\pm 0.49$} & \textbf{72.76} \tiny{$\pm 0.54$} \\
                     % & + \textbf{TAM} + \textbf{RKC}
                     % & 71.89 \tiny{$\pm 0.61$} & \textbf{71.58} \tiny{$\pm 0.65$} 
                     % & \textbf{59.12} \tiny{$\pm 0.83$} & \textbf{58.27} \tiny{$\pm 0.89$} 
                     % & \textbf{73.81} \tiny{$\pm 0.42$} & \textbf{73.24 } \tiny{$\pm 0.50$} \\
\bottomrule
\end{tabular}
}
\end{scriptsize}
\end{center}
\label{tb:integration_homo}
\vspace{-0.05in}
\end{table*}

